KEWS: A KPIs-Based Evaluation Framework of Workload Simulation On Microservice System

Simulating the workload is an essential procedure in microservice systems as it helps augment realistic workloads whilst safeguarding user privacy. The efficacy of such simulation depends on its dynamic assessment. The straightforward and most efficient approach to this is comparing the original workload with the simulated one using Key Performance Indicators (KPIs), which capture the state of the system. Nonetheless, due to the extensive volume and complexity of KPIs, fully evaluating them is not feasible, and measuring their similarity poses a significant challenge. This paper introduces a similarity metric algorithm for KPIs, the Extended Shape-Based Distance (ESBD), which gauges similarity in both shape and intensity. Additionally, we propose a KPI-based Evaluation Framework for Workload Simulations (KEWS), comprising three modules: preprocessing, compression, and evaluation. These methodologies effectively counteract the adverse effects of KPIs' characteristics and offer a holistic evaluation. Experimental results substantiate the effectiveness of both ESBD and KEWS.

==> CSCWD/content/relatedwork.tex <==
\section{Related Work}
In this section, we briefly review prior work on the KPI similarity metric. Then, we review workload simulation quality evaluation methods. Finally, we provide a summary of comparisons between the proposed method and its related work.

\subsection{KPI Similarity Metric}

The KPI is a time series which can be expressed as $\{t_1:x_1,t_2:x_2,t_3:x_3,...,t_m:x_m\}$, where $t_i$ denotes the timestamp, $x_i$ denotes the value of the corresponding timestamp and m is the length of the time series. In this paper, we do not consider the evaluation of the timestamp ${t_i}$ sequence and denote a certain metric by $\vec{x}=\{x_1,x_2,x_3,....x_m\}$.

Time series similarity can be used as an absolute criterion for making statistical inferences about the relationships between time series in different datasets and as a relative criterion for providing decisions in time series classification/clustering tasks\cite{lhermitte2011comparison}. In the past, many time series similarity metrics have been proposed in these two areas of research. Different time series similarity metrics have also been extensively compared\cite{serra2014empirical}\cite{wang2013experimental}. Time series similarity metrics are mainly classified into two categories\cite{lhermitte2011comparison}:(i) original time series similarity metrics and (ii) feature-based similarity metrics.

The similarity metric of the original time series directly utilises the original feature $\{x_i\}_{i=1}^m$ as the metric. The Minkowski distance ($L_n$ norm) is the simplest and most commonly used similarity metric, which generalises both the Manhattan distance ($L_1$) and the Euclidean distance ($L_2$). However, this lock-step metric is limited to equal-length sequences, cannot handle the phase shift of features, and is very sensitive to noise. Dynamic Time Warping (DTW)\cite{berndt1994using} is also a metric based on the $L_n$ norm, but it mitigates the phase shift of the features (time axis warping) by finding the best alignment through dynamic programming. As DTW has gradually become a major benchmark for time series similarity metrics, many variations of DTW methods have emerged\cite{lines2015time}, such as Weighted Dynamic Time Warping (WDTW)\cite{jeong2011weighted}, and Time Warp Edit Distance (TWED)\cite{marteau2008time}. Methods that compute similarity scores based on matching thresholds, such as the Longest Common Subsequence (LCSS)\cite{vlachos2002discovering}, Edit Distance with Real Penalty (ERP)\cite{chen2004marriage}, and Edit Distance on Real sequence (EDR)\cite{chen2005robust}, are still robust in the presence of noise and phase shifts. Unlike the metrics based on the $L_n$ norm, the correlation-based metric measures the linear relationship between the time series, rather than evaluates the differences in the values of the time series, which makes itself robust to amplitude deflation, noise and phase shifts and characterises the similarity of the time series in terms of a finite number of values, classical methods include Pearson's correlation number\cite{lee1988thirteen} and Shape-based Distance (SBD)\cite{paparrizos2015k}. However, 

The feature-based similarity metric maps the original feature $\{x_i\}_{i=1}^m\in\mathbb{R}^m$ into a feature space of lower dimensions, takes the feature vector $\{v_i\}_{i=1}^d\in\mathbb{R}^d$ as the object of the metric, then characterises the similarity of the original time series in terms of the similarity of the feature vectors. In this way, the dimension of the time series is reduced to cut off the computational cost and noise interference while preserving certain characteristics of the time series, but inevitably leading to information loss. In practice, it is a tedious task to choose an appropriate feature extraction method to trade off quality and efficiency. Classical time series feature extraction methods\cite{ding2008querying} are based on segmental discontinuous function approximation, such as Discrete Wavelet Transformation (DWT)\cite{chan1999efficient}, Piecewise Aggregate Approximation (PAA)\cite{keogh2001dimensionality}, and Methods based on low-order continuous polynomial approximation, such as Discrete Fourier Transformation (DFT)\cite{faloutsos1994fast}, Single Value Decomposition (SVD)\cite{ravi1998dimensionality} and so on. 

Recently, learning-based methods have emerged as successful methods of time series characterisation. Baydogan\cite{baydogan2016time} proposed a Learned Pattern Similarity (LPS) time series similarity measure. By modelling the relationships between time series segments, a tree-based learning strategy is used to discover dependency patterns, a bag-of-words pattern is used to encode a representation of the dependency patterns and a pattern-matching similarity metric is designed based on this representation. To cope with the challenges of long time series and sparse data labels, Franceschi\cite{franceschi2019unsupervised} proposed an unsupervised method to learn a generic representation of multivariate time series. The method combines an encoder based on causally dilated convolution and a ternary loss based on time-negative sampling. Zerveas\cite{zerveas2021transformer} proposed a Transfomer-based framework for learning multivariate time series representations. It extracts dense vectorial representations of multivariate time series from denoised targets by training Transformer encoders with unlabelled data. TS2Vec\cite{yue2022ts2vec} proposed a general framework for learning time series representations at arbitrary semantic levels. TS2Vec learns the augmented contextual views hierarchically in contrast to each other, and obtains, by aggregating timestamps, the representations of arbitrary subsequences in time series. 

\subsection{Workload Simulation Quality Evaluation}

Since it is difficult to retrieve relevant studies on quality evaluation of workload simulation, the key to quality evaluation of workload simulation lies in how to select appropriate KPIs for evaluation from a large amount of KPIs data, i.e., to achieve the compression of the KPIs evaluation set\cite{peiris2014pad}. In this paper, the research on workload simulation quality evaluation method focuses on the scale compression of KPIs data. The complex architecture of microservice systems makes the topological relationships between different system elements diverse. As a result, there are usually GG, and key homogeneous KPIs can be extracted through domain knowledge or KPIs clustering to achieve KPIs evaluation set compression.

Nowadays, most microservice applications follow certain microservice design paradigms\cite{dragoni2017microservices} and deploy several tools to monitor the state information of the system\cite{waseem2021design}, such as Prometheus, Elasticsearch, and so on. Halawa\cite{halawa2020unsupervised} qualitatively identified explicit correlations among KPIs through domain knowledge and used it as a priori to guide KPI clustering. Peral\cite{peral2017application} semi-automatically and quantitatively determined the correlation between KPIs and target business using data mining-related techniques. 
Chaos engineering\cite{basiri2016chaos} proposed by Netflix Company in 2017 is an experimental method for verifying the ability of microservice systems to cope with failures, and its core idea is to introduce disturbing variables reflecting real-world events in production environments and to show the system's ability to cope with failures by comparing and analysing the before-and-after differences of the system's homeostasis. Yin\cite{Yin2021microservice} proposed a method to identify and analyse the resilience risk of a system by using multiple service performance indicators to jointly indicate the system's homeostasis, identify the system's resilience risk by analysing the homeostatic deviation of each indicator in chaotic experiments, and analyse the causality of service performance indicators by constructing causality diagrams. Meanwhile, they pointed out that service performance indicators have different steady-state baselines and offset responses to fault perturbations. 
Su\cite{su2019coflux} proposed an unsupervised method, CoFlux, to reveal the correlations among KPIs under anomalous conditions.CoFlux extracts the fluctuation features (prediction errors) by combining the KPIs prediction models, characterises the correlations among KPIs in terms of the correlations of the fluctuation features, and applies them to alarm compression, root cause recommendation, and fluctuation propagation construction, which effectively assists in the troubleshooting of service anomalies.

KPIs clustering is a research subset of time series clustering algorithms. Compared with ideal time series, KPIs have more complex characteristics. Therefore, commonly used time series clustering algorithms, such as segmentation clustering, hierarchical clustering, density clustering, etc.\cite{jeong2011weighted}, cannot be directly applied to indicator data. 
Yahyaoui\cite{yahyaoui2018unsupervised} proposed a clustering method based on the long-term change of KPIs. The method uses information entropy weights to aggregate KPIs.Then, features of the aggregated KPIs are extracted using the Harr wavelet transform. Finally, internal evaluation metrics (e.g., profile coefficients and Dunn's index) are used to determine the optimal estimation of the number of clusters and the optimal selection of clustering algorithms. 

Since anomalous KPIs usually distort the clustering results, KADT\cite{qian2020large} proposed a fast clustering method for KPIs, which combines random downsampling, sliding window and K-Shape to extract the KPIs' curve patterns to isolate the anomalous KPIs' curve patterns, and constructs a model for detecting KPIs' anomalies through the centre of mass of the KPIs' curve patterns. 

To reduce the training overhead of the KPIs anomaly detection model, AnoTransfer\cite{zhang2022efficient} proposed a KPI clustering method based on variational autoencoder, training the variational autoencoder to extract the KPI segment features, uses hierarchical clustering combined with the Euclidean distance to cluster the KPI segment features, and applies the clustering centre of gravity to the anomaly detection model migration learning. 

Halawa\cite{halawa2020unsupervised} proposed another KPI clustering algorithm based on hierarchical clustering. The dimensionality of KPI data was reduced by a fixed PCA algorithm with two principal components, and its accuracy was verified in the CESGA real dataset using a bottom-up hierarchical clustering algorithm based on different similarity metrics. 

Guo\cite{guo2016clustering} proposed a KPI density clustering method based on CFSFDP\cite{rodriguez2014clustering}. Based on the assumption of strong linear correlation among KPIs, KPI clusters are divided by CFSFDP and linear equations are fitted inside the clusters using regression methods to clarify the implied linear correlations among KPIs. 

ROCKA\cite{li2018robust} proposed a robust and fast KPI clustering method, which extracts the KPI base shapes by using moving averages, heuristically estimates the density by the k-nearest-neighbour distance map smoothing region radius, and the DBSCAN\cite{ester1996density} algorithm is used to accurately and quickly divide the KPI clusters. 

TPC\cite{wang2021rapid} proposed an improved KPIs clustering method based on ROCKA, which optimises the selection method of ROCKA density radius estimation: the candidate inflexion point instead of the maximum candidate is used as the optimal density radius estimation, thus obtaining more accurate clustering results in complex data. In anomaly detection scenarios, the goal of KPIs clustering is to improve the accuracy of anomaly detection rather than to obtain accurate clustering results. For this reason, 

DDCOL\cite{yu2019unsupervised} proposed another KPI clustering method based on DBSCAN and designed a heuristic density radius estimation algorithm which is more suitable for anomaly detection. The core idea is to find the inflexion point of the k-nearest-neighbour distance curve.

\textit{Comparisons with related graph CL methods.} In summary, we provide a brief comparison between the proposed GCA and other state-of-the-art graph contrastive representation learning methods, including DGI [45], GMI [32], and MVGRL [16] in Table 1, where the last two columns denote data augmentation strategies at topology and attribute levels respectively. It is seen that the proposed GCA method simplifies the previous node–global contrastive scheme by defining contrastive objective at the node level. Most importantly, GCA is the only one that proposes adaptive data augmentation on both topology and attribute levels.
